AutoGrow: Automatic Layer Growing in Deep Convolutional Networks

Depth is a key component of Deep Neural Networks (DNNs), however, designing depth is heuristic and requires many human efforts. We propose AutoGrow to automate depth discovery in DNNs: starting from a shallow seed architecture, AutoGrow grows new layers if the growth improves the accuracy; otherwise, stops growing and thus discovers the depth. We propose robust growing and stopping policies to generalize to different network architectures and datasets. Our experiments show that by applying the same policy to different network architectures, AutoGrow can always discover near-optimal depth on various datasets of MNIST, FashionMNIST, SVHN, CIFAR10, CIFAR100 and ImageNet. For example, in terms of accuracy-computation trade-off, AutoGrow discovers a better depth combination in ResNets than human experts. Our AutoGrow is efficient. It discovers depth within similar time of training a single DNN. Our code is available at https://github.com/wenwei202/autogrow.

==> tables/autogrow-adaptation-minipage.tex <==
\centering
\resizebox{.7\columnwidth}{!}{
 	\begin{tabular}{llllr}
 		\toprule
 		net & dataset &  found net & accu \%  & $\Delta$\textsuperscript{$*$} \\
 		\midrule 
 		\multirow{5}{*}{\texttt{Basic3ResNet}} & CIFAR10  & \texttt{42-42-42} & 94.27 & -0.03 \\
 		%\parbox[t]{2mm}{\multirow{5}{*}{\rotatebox[origin=c]{45}{\texttt{Basic3ResNet}}}} & CIFAR10  & \texttt{} &  & \\
 		& CIFAR100  & \texttt{54-53-53} & 74.72 & \textbf{-0.95} \\
 		& SVHN  & \texttt{34-34-34} & 97.22 & 0.04 \\
 		& FashionMNIST  & \texttt{30-29-29} & 94.57 &  -0.06 \\
 		& MNIST  & \texttt{33-33-33} & 99.64 & -0.03 \\ 
 		
 		\midrule 
 		\multirow{5}{*}{\texttt{Basic4ResNet}} & CIFAR10  & \texttt{22-22-22-22} & 95.49 & -0.10 \\
 		%\parbox[t]{2mm}{\multirow{5}{*}{\rotatebox[origin=c]{45}{\texttt{Basic3ResNet}}}} & CIFAR10  & \texttt{} &  & \\
 		& CIFAR100  & \texttt{17-51-16-16} & 79.47 & \textbf{1.22} \\
 		& SVHN  & \texttt{20-20-19-19} & 97.32 & -0.08 \\
 		& FashionMNIST  & \texttt{27-27-27-26} & 94.62 & \textbf{-0.17}\\
 		& MNIST  & \texttt{11-10-10-10} & 99.66 & 0.01 \\ 
 		
 		\midrule 
 		\multirow{5}{*}{\texttt{Plain3Net}} & CIFAR10  & \texttt{23-22-22} & 90.82 & \textbf{6.49}\\
 		%\parbox[t]{2mm}{\multirow{5}{*}{\rotatebox[origin=c]{45}{\texttt{Basic3ResNet}}}} & CIFAR10  & \texttt{} &  & \\
 		& CIFAR100  & \texttt{28-28-27} & 66.34 & \textbf{31.53} \\
 		& SVHN  & \texttt{36-35-35} & 96.79 & \textbf{77.20} \\
 		& FashionMNIST  & \texttt{17-17-17} & 94.49 & \textbf{0.56} \\
 		& MNIST  & \texttt{20-20-20} & 99.66 & \textbf{0.12} \\ 
 		
 		
 		\midrule 
 		\multirow{5}{*}{\texttt{Plain4Net}} & CIFAR10  & \texttt{17-17-17-17} & 94.20 & \textbf{5.72} \\
 		%\parbox[t]{2mm}{\multirow{5}{*}{\rotatebox[origin=c]{45}{\texttt{Basic3ResNet}}}} & CIFAR10  & \texttt{} &  & \\
 		& CIFAR100  & \texttt{16-15-15-15} & 73.91 & \textbf{29.34} \\
 		& SVHN  & \texttt{12-12-12-11} & 97.08 & \textbf{0.32} \\
 		& FashionMNIST  & \texttt{13-13-13-13} & 94.47 & \textbf{0.72} \\
 		& MNIST  & \texttt{13-12-12-12} & 99.57 & 0.03 \\ 
 		
 		
 		
 		\bottomrule
 		\multicolumn{5}{l}{\textsuperscript{$*$} $\Delta = $ (accuracy of \autogrow{}) $-$ (accuracy of training from scratch) }
 	\end{tabular}
}
\label{tab:autogrow-adaptation-minipage}
\captionof{table}{ The adaptability of \autogrow{} to datasets}

==> tables/autogrow-after-convergence.tex <==
\begin{table}
  \caption{ Growing before convergence under initializers }
  \label{tab:autogrow-morphism}
  \centering
  \resizebox{1.0\columnwidth}{!}{
  	\begin{tabular}{cccccc}
  		\toprule
  		dataset & optimizer &  initializer & found net & accu \%  & $\Delta$ \\
  		\midrule 
  		\multirow{4}{*}{CIFAR10}& sgd  & \texttt{ZeroInit} & 2-2-4 & 92.23  & 0.16\\
  		& sgd  & \texttt{AdamInit} & 3-4-4 &  92.60 & -0.41 \\ 
  		& sgd  & \texttt{UniInit} & 3-4-4 & 92.93  & -0.08\\
  		& sgd  & \texttt{GauInit} & 2-4-3 & 93.12  & 0.55\\
  		
  		\midrule 
  		
  		\multirow{4}{*}{CIFAR100} & sgd  & \texttt{ZeroInit} & 3-2-4 & 70.22   &  0.35\\
  		& sgd  & \texttt{AdamInit} & 3-3-3 & 69.70 & -0.80 \\
  		& sgd  & \texttt{UniInit} & 4-4-3 & 70.39   & 0.36 \\
  		& sgd  & \texttt{GauInit} & 3-4-3 & 70.66 & 0.91\\
  		
  		\bottomrule
  		%\multicolumn{3}{l}{\textsuperscript{$\dagger$} SVD and k-means preserve the same ranks with PCA }
  	\end{tabular}
  }
\end{table} 

==> tables/autogrow-imagenet-update.tex <==
\begin{table}[h]
  % \caption{ Scaling up to ImageNet}
  \vspace{-10pt}
  \label{tab:autogrow-imagenet}
  \centering
  \resizebox{1.\columnwidth}{!}{
  	\begin{tabular}{llllcc}
  		\toprule
  		net & $K$ &  found net & Top-1  & Top-5 & \textsuperscript{$\dagger$}$\Delta$ Top-1  \\
  		\midrule 
  		\multirow{2}{*}{\texttt{Basic4ResNet}} & 2 & \texttt{12-12-11-11} & 76.28 & 92.79 & 0.43 \\
  		 & 5  & \texttt{9-3-6-4} & 74.75 & 91.97 & 0.72 \\
  		 
  		 \midrule 
  		 \multirow{2}{*}{\texttt{Bottleneck4ResNet}} & 2 & \texttt{6-6-6-17} & 77.99  & 93.91 & \yc{\textbf{0.83 }}\\
  		 & 5  & \texttt{6-7-3-9} & 77.33 & 93.65 & 0.83 \\
  		 
  		 \midrule 
  		 \multirow{2}{*}{\texttt{Plain4Net}} & 2 & \texttt{6-6-6-6} & 71.22  & 90.08 & 0.70\\
  		 & 5  & \texttt{5-5-5-4} & 70.54 & 89.76 & 0.93 \\
  		 
  		
  		\bottomrule
  		\multicolumn{5}{l}{\textsuperscript{$\dagger$} $\Delta = $ (Top-1 of \autogrow{}) $-$ (Top-1 of training from scratch) }
  	\end{tabular}
  }
\vspace{-6pt}
\end{table} 
